Latent Reasoning VLA: Latent Thinking and Prediction for Vision-Language-Action Models

Vision-Language-Action (VLA) models benefit from chain-of-thought (CoT) reasoning, but existing approaches incur high inference overhead and rely on discrete reasoning representations that mismatch continuous perception and control. We propose Latent Reasoning VLA (LaRA-VLA), a unified VLA framework that internalizes multi-modal CoT reasoning into continuous latent representations for embodied action. LaRA-VLA performs unified reasoning and prediction in latent space, eliminating explicit CoT generation at inference time and enabling efficient, action-oriented control. To realize latent embodied reasoning, we introduce a curriculum-based training paradigm that progressively transitions from explicit textual and visual CoT supervision to latent reasoning, and finally adapts latent reasoning dynamics to condition action generation. We construct two structured CoT datasets and evaluate LaRA-VLA on both simulation benchmarks and long-horizon real-robot manipulation tasks. Experimental results show that LaRA-VLA consistently outperforms state-of-the-art VLA methods while reducing inference latency by up to 90\% compared to explicit CoT-based approaches, demonstrating latent reasoning as an effective and efficient paradigm for real-time embodied control. Project Page: https://loveju1y.github.io/Latent-Reasoning-VLA/

==> figures/latent_collapse.tex <==
\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=0.495\textwidth]{imgs/latent_collapse.pdf}}
\caption{
Latent collapse analysis.
}
\label{fig: latent_collapse}
\end{center}
\end{figure}

==> tables/bridge_para.tex <==
\begin{table}[htbp]
\centering
\small
\caption{Hyperparameter settings for SimplerEnv experiments.}
\label{tab:simpler_params}
\begin{tabular}{l c c c}
\toprule
Hyperparameters & Stage I & Stage II & Stage III \\
\midrule
\multicolumn{4}{l}{\textit{Learning Rates}} \\
\quad VLM LR & $1 \times 10^{-5}$ & $1 \times 10^{-5}$ & $1.3 \times 10^{-5}$ \\
\quad DiT LR & $1 \times 10^{-4}$ & $1 \times 10^{-4}$ & $1.3 \times 10^{-4}$ \\
\midrule
\multicolumn{4}{l}{\textit{Optimization Config}} \\
\quad Action Horizon & 16 & 16 & 16 \\
\quad Training Steps & 10k & 5k / 5k / 10k & 60k \\
\quad Batch Size & 12 & 16 & 16 \\
\quad Optimizer & AdamW & AdamW & AdamW \\
\quad LR Scheduler & Cosine (Min. LR) & Cosine (Min. LR) & Cosine (Min. LR) \\
\quad Warm-up Ratio & 0.1 & 0.1 & 0.1 \\
\midrule
\multicolumn{4}{l}{\textit{Loss Weights}} \\
\quad Action Token Loss & 1.0 & 1.0 & -- \\
\quad Image Next Loss & 0.1 & 0.2 & -- \\
\quad CoT Loss & 1.0 & 1.0 & -- \\
\quad DiT Loss & -- & -- & 1.0 \\
\bottomrule
\end{tabular}
\vskip -0.1in
\end{table}

==> tables/libero_para.tex <==
\begin{table}[htbp]
\centering
\small
\caption{Hyperparameter settings for LIBERO experiments.}
\label{tab:libero_params}
\begin{tabular}{l c c c}
\toprule
Hyperparameters & Stage I & Stage II & Stage III \\
\midrule
\multicolumn{4}{l}{\textit{Learning Rates}} \\
\quad VLM LR & $1 \times 10^{-5}$ & $1 \times 10^{-5}$ & $1 \times 10^{-5}$ \\
\quad DiT LR & $1 \times 10^{-4}$ & $1 \times 10^{-4}$ & $1 \times 10^{-4}$ \\
\midrule
\multicolumn{4}{l}{\textit{Optimization Config}} \\
\quad Action Horizon & 8 & 8 & 8 \\
\quad Training Steps & 5k & 2k / 2k / 2k & 40k \\
\quad Batch Size & 12 & 16 & 16 \\
\quad Optimizer & AdamW & AdamW & AdamW \\
\quad LR Scheduler & Cosine (Min. LR) & Cosine (Min. LR) & Cosine (Min. LR) \\
\quad Warm-up Ratio & 0.1 & 0.1 & 0.1 \\
\midrule
\multicolumn{4}{l}{\textit{Loss Weights}} \\
\quad Action Token Loss & 1.0 & 1.0 & -- \\
\quad Image Next Loss & 0.1 & 0.2 & -- \\
\quad CoT Loss & 1.0 & 1.0 & -- \\
\quad DiT Loss & -- & -- & 1.0 \\
\bottomrule
\end{tabular}
\vskip -0.1in
\end{table}

==> tables/realworld_para.tex <==
\begin{table}[htbp]
\centering
\small
\caption{Hyperparameter settings for Real Robot experiments.}
\label{tab:real_robot_params}
\begin{tabular}{l c c c}
\toprule
Hyperparameters & Stage I & Stage II & Stage III \\
\midrule
\multicolumn{4}{l}{\textit{Learning Rates}} \\
\quad VLM LR & $1 \times 10^{-5}$ & $1 \times 10^{-5}$ & $1 \times 10^{-5}$ \\
\quad DiT LR & $1 \times 10^{-4}$ & $1 \times 10^{-4}$ & $1 \times 10^{-4}$ \\
\midrule
\multicolumn{4}{l}{\textit{Optimization Config}} \\
\quad Action Horizon & 25 & 25 & 25 \\
\quad Training Steps & 5k & 2k / 2k / 2k & 10k \\
\quad Batch Size & 12 & 16 & 16 \\
\quad Optimizer & AdamW & AdamW & AdamW \\
\quad LR Scheduler & Cosine (Min. LR) & Cosine (Min. LR) & Cosine (Min. LR) \\
\quad Warm-up Ratio & 0.1 & 0.1 & 0.1 \\
\midrule
\multicolumn{4}{l}{\textit{Loss Weights}} \\
\quad Action Token Loss & 1.0 & 1.0 & -- \\
\quad Image Next Loss & 0.1 & 0.2 & -- \\
\quad CoT Loss & 1.0 & 1.0 & -- \\
\quad DiT Loss & -- & -- & 1.0 \\
\bottomrule
\end{tabular}
\vskip -0.1in
\end{table}
